Adversarial Style Augmentation via Large Language Model for Robust Fake News Detection

The spread of fake news harms individuals and presents a critical social challenge that must be addressed. Although numerous algorithmic and insightful features have been developed to detect fake news, many of these features can be manipulated with style-conversion attacks, especially with the emergence of advanced language models, making it more difficult to differentiate from genuine news. This study proposes adversarial style augmentation, AdStyle, designed to train a fake news detector that remains robust against various style-conversion attacks. The primary mechanism involves the strategic use of LLMs to automatically generate a diverse and coherent array of style-conversion attack prompts, enhancing the generation of particularly challenging prompts for the detector. Experiments indicate that our augmentation strategy significantly improves robustness and detection performance when evaluated on fake news benchmark datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tables/full_result.tex <==
% \begin{table*}[t!]
% \caption{Performance comparison with \model{} in four different style—conversion attacks. For the attack scenario, we report the AUC of four style-conversion attacks. Our model demonstrates a significant performance improvement over all text-based fake news detectors in diverse style-conversion attack scenarios.  (NY: The New York Times, TS: The Sun, NE:  National Enquirer ) \looseness=-1}
% \centering
% \scalebox{1.1}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{CNN} &  & Politifact  & &  &  Gossipcop& &  &Constraint & \\
%  & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 \\
% \midrule
% Vanilla & 0.5664 & 0.6566 & 0.8127 & 0.6841 & 0.7913 & 0.8518 & 0.8563 & 0.8175 & 0.8056 \\
% UDA & 0.5906 & 0.7174 & 0.8009 & 0.7294 & 0.7859 & 0.8599 & 0.8305 & 0.8594 & 0.9021 \\
% RADAR & 0.7205 & 0.7301 & 0.7926 & 0.7683 & 0.8138 & 0.8666 & 0.8099 & 0.8400 & 0.8873 \\
% ENDEF & 0.5426 & 0.6679 & 0.7588 & 0.7288 & 0.7839 & 0.8624 & 0.7695 & 0.8666 & 0.8353 \\
% SheepDog & 0.6305 & 0.8269 & 0.8683 & 0.7472 & 0.8393 & 0.8706 & 0.9200 & 0.9022 & 0.9544 \\ \midrule
% \model{}  & 0.7547 & 0.8822 & 0.9174 & 0.8195 & 0.8429 & 0.8744 & 0.9344 & 0.9430 & 0.9646 \\
% \bottomrule
% \end{tabular}
% }


% \vspace{1.0mm}

% \scalebox{1.1}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{NY} &  & Politifact & &  &  Gossipcop& &  & Constraint & \\
%  & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 \\
% \midrule
% Vanilla & 0.5899 & 0.7334 & 0.8687 & 0.6750 & 0.7797 & 0.8465 & 0.8522 & 0.8939 & 0.8868 \\
% UDA & 0.6189 & 0.7644 & 0.8744 & 0.7207 & 0.7795 & 0.8558 & 0.8745 & 0.9184 & 0.9297 \\
% RADAR & 0.6966 & 0.7853 & 0.8586 & 0.7481 & 0.7960 & 0.8574 & 0.8701 & 0.8974 & 0.9176 \\
% ENDEF & 0.6152 & 0.7630 & 0.8150 & 0.7227 & 0.7837 & 0.8609 & 0.8341 & 0.9067 & 0.8918 \\
% SheepDog & 0.6310 & 0.7990 & 0.9090 & 0.7420 & 0.8309 & 0.8650 & 0.8937 & 0.9254 & 0.9645 \\ \midrule
% \model{} & 0.7599 & 0.8940 & 0.9444 & 0.8118 & 0.8389 & 0.8686 & 0.9243 & 0.9594 & 0.9720 \\
% \bottomrule
% \end{tabular}
% }
% \vspace{1.0mm}

% \scalebox{1.1}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{TS} &  & Politifact  & &  &  Gossipcop& &  &Constraint & \\
%  & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 \\
% \midrule
% Vanilla & 0.6913 & 0.6859 & 0.8789 & 0.7068 & 0.7918 & 0.8430 & 0.7822 & 0.8727 & 0.8974 \\
% UDA & 0.6646 & 0.8072 & 0.8883 & 0.7488 & 0.7904 & 0.8613 & 0.8662 & 0.9145 & 0.9446 \\
% RADAR & 0.7271 & 0.7173 & 0.8909 & 0.7594 & 0.8062 & 0.8620 & 0.8564 & 0.8882 & 0.9132 \\
% ENDEF & 0.7001 & 0.8132 & 0.8444 & 0.7603 & 0.7909 & 0.8639 & 0.8445 & 0.8955 & 0.9043 \\
% SheepDog & 0.7070 & 0.8408 & 0.9096 & 0.7580 & 0.8395 & 0.8688 & 0.8962 & 0.9217 & 0.9665 \\ \midrule
% \model{} & 0.8444 & 0.9002 & 0.9520 & 0.8117 & 0.8347 & 0.8751 & 0.9219 & 0.9521 & 0.9727 \\
% \bottomrule
% \end{tabular}
% }

% \vspace{1.0mm}

% \scalebox{1.1}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{NE} &  & Politifact  & &  &  Gossipcop& &  &Constraint & \\
%  & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 & 0.1 & 0.25 & 1 \\
% \midrule
% Vanilla & 0.6432 & 0.6856 & 0.8591 & 0.7020 & 0.7875 & 0.8399 & 0.7833 & 0.8853 & 0.9067 \\
% UDA & 0.6557 & 0.7892 & 0.8622 & 0.7450 & 0.7902 & 0.8595 & 0.8747 & 0.9191 & 0.9423 \\
% RADAR & 0.7428 & 0.7269 & 0.8864 & 0.7573 & 0.8026 & 0.8556 & 0.8775 & 0.8919 & 0.9161 \\
% ENDEF & 0.6924 & 0.7877 & 0.8355 & 0.7502 & 0.7897 & 0.8589 & 0.8456 & 0.9112 & 0.9025 \\
% SheepDog & 0.6636 & 0.8268 & 0.9166 & 0.7521 & 0.8331 & 0.8632 & 0.8606 & 0.9257 & 0.9667 \\ \midrule
% \model{} & 0.8029 & 0.8913 & 0.9460 & 0.8166 & 0.8391 & 0.8702 & 0.9092 & 0.9579 & 0.9771 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:style_attack_full_result}
% \end{table*}



